TextCaps : Handwritten Character Recognition with Very Small Datasets

Many localized languages struggle to reap the benefits of recent advancements in character recognition systems due to the lack of substantial amount of labeled training data. This is due to the difficulty in generating large amounts of labeled data for such languages and inability of deep learning techniques to properly learn from small number of training samples. We solve this problem by introducing a technique of generating new training samples from the existing samples, with realistic augmentations which reflect actual variations that are present in human hand writing, by adding random controlled noise to their corresponding instantiation parameters. Our results with a mere 200 training samples per class surpass existing character recognition results in the EMNIST-letter dataset while achieving the existing results in the three datasets: EMNIST-balanced, EMNIST-digits, and MNIST. We also develop a strategy to effectively use a combination of loss functions to improve reconstructions. Our system is useful in character recognition for localized languages that lack much labeled training data and even in other related more general contexts such as object recognition.

==> figures/overall.tex <==
%\usetikzlibrary{matrix}
\begin{tikzpicture}[x=0.7cm, y=0.7cm, every node/.append style={text=black, font=\scriptsize}]

	  \matrix (m) [matrix of nodes,
    column sep=0.2cm,
    row sep=-0.2cm,
    nodes={draw, % General options for all nodes
      anchor=center,
      text centered,
      %rounded corners,
      %minimum width=1.5cm,
      minimum height=8mm
    },
    % Define styles for some special nodes
    right iso/.style={isosceles triangle,scale=0.5,sharp corners, anchor=center, xshift=-4mm},
    left iso/.style={right iso, rotate=180, xshift=-8mm},
    txt/.style={text width=1.5cm,anchor=center},
    ellip/.style={ellipse,scale=0.5},
    empty/.style={draw=none}
    ]
  {
  %Row 1
   &   \begin{tikzpicture} \draw (-0.1,-0.3) rectangle ++(0.5,0.5); \draw (0.6,0.6) rectangle ++(0.4, -0.4);
  \draw (0.8,0.3) rectangle ++(0.4, -0.4);
  \draw (1.2,-0.3) rectangle ++(0.4, -0.4);
  \draw (2, 0.3) rectangle ++(0.3, -0.8);
  \draw[-latex] (0.4, -0.05) -- ++(0.3, 0);
  \end{tikzpicture} & Addition &  &
  \begin{tikzpicture}
  	\draw[-latex] (0,0) -- (2.5,0);
  	\draw[-latex] (0,0) -- (0,2);  	
  	\foreach \i/\h/\c in {1/0.6/{rgb:red,4;green,2;yellow,1},2/0.8/{rgb:red,1;green,2;yellow,1},3/1.2/{rgb:red,4;green,1;yellow,1},4/1.5/{rgb:red,1;green,1;blue,4},5/0.8/{rgb:red,4;magenta,4;yellow,1},6/0.5/{rgb:red,1;green,1;yellow,3}}
  	{
  		\draw[fill={\c}] (0.3*\i, 0) rectangle ++(0.3, \h);
  	}
  \end{tikzpicture}
  &  &  & \\
$v_{i,1}$ & & & & & Fusion layer&

  \begin{tikzpicture}
  	\draw[-latex] (0,0) -- (2.5,0);
  	\draw[-latex] (0,0) -- (0,2);  	
  	\foreach \i/\h/\c in {1/0.56/{rgb:red,4;green,2;yellow,1},2/0.72/{rgb:red,1;green,2;yellow,1},3/1.32/{rgb:red,4;green,1;yellow,1},4/1.42/{rgb:red,1;green,1;blue,4},5/0.76/{rgb:red,4;magenta,4;yellow,1},6/0.42/{rgb:red,1;green,1;yellow,3}}
  	{
  		\draw[fill={\c}] (0.3*\i, 0) rectangle ++(0.3, \h);
  	}
  \end{tikzpicture}

 \\
%Row 3
&
\begin{tikzpicture}
	\draw[fill=red!40] (0,0) coordinate (a) -- ++(0.2, -0.1) coordinate (b) -- ++(0.1, 0.15) coordinate (c) -- ++(-0.2, 0.1) coordinate (d) -- cycle;
	\draw[fill=blue!40]  (0,-0.5) coordinate (i) -- ++(0.2, -0.1) coordinate (j) -- ++(0.1, 0.15) coordinate (k) -- ++(-0.2, 0.1) coordinate (l) -- cycle;
	\begin{scope}[xshift=50, yshift=5]
		\draw[fill=red!60]  (0,0) coordinate (e) -- ++(0.2, -0.1) coordinate (f) -- ++(0.1, 0.15) coordinate (g) -- ++(-0.2, 0.1) coordinate (h) -- cycle;
		\draw[fill=blue!60]  (0,-1) coordinate (m) -- ++(0.2, -0.1) coordinate (n) -- ++(0.1, 0.15) coordinate (o) -- ++(-0.2, 0.1) coordinate (p) -- cycle;		
	\end{scope}
	\draw[dashed] (a) .. controls (0.5,0.5) ..  (e);
	\draw (b) .. controls (0.7,0.4) ..  (f);
	\draw (c) .. controls (0.8,0.55) ..  (g);
	\draw (d) .. controls (0.6,0.65) ..  (h);
	
	\draw[dashed] (i) .. controls (0.5,-0.3) ..  (m);
	\draw (j) .. controls (0.7,-0.4) ..  (n);
	\draw (k) .. controls (0.8, -0.25) ..  (o);
	\draw (l) .. controls (0.6, -0.15) ..  (p);	
\end{tikzpicture}
& \begin{tikzpicture}
	\draw (0,0) circle (1);
	\foreach \a in {0, 1, 2, 3, 4, 5}
	{
		\draw (\a*30:1) -- ++(\a*30:-2);
	}
\end{tikzpicture} &
BoW &
  \begin{tikzpicture}
  	\draw[-latex] (0,0) -- (2.5,0);
  	\draw[-latex] (0,0) -- (0,2);  	
  	\foreach \i/\h/\c in {1/0.5/{rgb:red,4;green,2;yellow,1},2/0.6/{rgb:red,1;green,2;yellow,1},3/1.5/{rgb:red,4;green,1;yellow,1},4/1.3/{rgb:red,1;green,1;blue,4},5/0.7/{rgb:red,4;magenta,4;yellow,1},6/0.3/{rgb:red,1;green,1;yellow,3}}
  	{
  		\draw[fill={\c}] (0.3*\i, 0) rectangle ++(0.3, \h);
  	}
  \end{tikzpicture}
\\

$v_{i,n}$ & & & & & & & &

\begin{tikzpicture}[scale=0.3]
	\draw  (0,0) -- ++(2, 0) -- ++(0, 0.5) coordinate  (a)  -- ++(-4, 0) coordinate  (b) -- ++(0, -0.5) -- cycle;
	
	
	\draw  (0,2) -- ++(3, 0) coordinate  (c) -- ++(0, 0.5) coordinate (d)  -- ++(-6, 0) coordinate  (e) -- ++(0, -0.5)  coordinate  (f)  -- cycle;
	
	\draw  (0,4) -- ++(1.5, 0)  coordinate  (g) -- ++(0, 0.5)  -- ++(-3, 0) coordinate[midway] (t) -- ++(0, -0.5) coordinate  (h) -- cycle;	
	
	\draw[-latex] (a) -- (f);
	\draw[-latex] (b) -- (c);
	
	\draw[-latex] (e) -- (g);
	\draw[-latex] (d) -- (h);	
	
	\draw[-latex] (t) -- ++(0, 1);		
	\draw[-latex] (e)  .. controls ++(-2,2) and ++(-2, -2) ..  (f);
\end{tikzpicture}
\\
  };

  \node at (m-1-2) [anchor=south, yshift=20] {CNN};
  \node at (m-3-3) [anchor=south, yshift=20] {HOOF};
    \node at (m-4-9) [anchor=south, yshift=20] {LSTM network};
        \node at (m-1-5) [anchor=south, yshift=20] {Static vector};
        \node at (m-3-5) [anchor=south, yshift=20] {Motion vector};
        \node at (m-3-2) [anchor=south, yshift=20] {Motion tubes};

  \draw[-latex] (m-2-1) |- (m-1-2);
  \draw[-latex] (m-2-1) |- (m-3-2);

    \draw[-latex] (m-1-2) -- (m-1-3);
  \draw[-latex] (m-3-2) -- (m-3-3);

   \draw[-latex] (m-1-3) --(m-1-5);
  \draw[-latex] (m-3-3) -- (m-3-4);
    \draw[-latex] (m-3-4) --  (m-3-5);

     \draw[-latex] (m-1-5) -| (m-2-6);
    \draw[-latex] (m-3-5) -|  (m-2-6);

\draw[-latex] (m-2-6) -- (m-2-7);

\draw[-latex] (m-2-7) |- ($(m-4-9.west)+(0, 0.8)$);
\draw[-latex] ($(m-4-9.west)+(-2.4, 0.4)$) -- ++(2.4, 0);
\draw[-latex] ($(m-4-9.west)+(-2.4, 0)$) -- ++(2.4, 0);
\node at ($(m-4-9.west)+(-2.4, -0.25)$) {$\vdots$};
\draw[-latex] ($(m-4-9.west)+(-2.4, -0.8)$) -- ++(2.4, 0);

\node at ($(m-4-1)+(0, 1.5)$) {$\vdots$};
\node at ($(m-4-1)+(5, 0)$) {$\cdots$};

\draw[-latex] (m-4-9) -- ++(2,0) node [anchor=west] {Classification};

\end{tikzpicture}

==> methodology_cnn.tex <==
\subsection{Comparison with CNN}
For the purpose of comparison, we propose a simple CNN architecture, comparable with the CapsNet architecture of the base model. However, it is important to note that CNN does not provide reconstruction capability as CapsNet, we evaluate this model only for comparison and completeness. The proposed CNN architecture consists of four main layers and designed to have maximum number of parameters possible with highest accuracy.

The first layer of the CNN is identical to the CapsNet base model, which is a convolutional layer with 256, 9x9 kernels with a stride of 1 and ReLU activation. The second layer is somewhat similar to the Primary Capsule layer in the base model, which has the same convolutional layer of 128, 9x9 kernels with a stride of 1 and ReLU activation, but followed by a pooling layer with filters of size 2x2 of max pooling. The third layer is designed to match the DigitCaps layer with a convolutional layer followed by a fully connected layer. This layer consists of a convolutional layer of 256, 3x3 kernels with a stride of 1 and ReLU activation, a pooling layer with filters of size 2x2 of max pooling, and a fully connected layer of 1024 outputs with ReLU activation. A flatten layer is added in between pooling and fully connected layers. 

Two fully connected layers are included in the fourth and final layer. The first fully connected layer outputs a vector of size 512 with ReLU activation and the output size of the final fully connected layer with sigmoid activation is the number of classes used. 

==> methodology_snapshot.tex <==
% \subsection{Snapshot Ensembling}
We use ensembling to improve our model accuracy. We use cyclic learning rates for each 30 epochs. this give us 3 ensemble models with 90 epochs as well as avoid the over fitting in the model.

==> methodology_variations.tex <==
\subsection{Variations to the Existing Architecture}
The current architecture proposed by \cite{sabour2017dynamic} for the MNIST dataset is a shallow architecture with 3 layers and 3 additional reconstruction layers. The first layer is a convolutional layer consisting 256, 9$\times$9 kernels with a stride of 1 and ReLU activation. The second layer is a convolutional capsule layer with 32 channels of 8-dimensional convolutional capsules, with each primary capsule containing 8 convolutional units with a 9$\times$9 kernel and a stride of 2. The third layer has a 16-dimensional capsule per class, resulting in 10 capsules for the MNIST dataset. 

The first two reconstruction layers are fully connected layers with ReLU activation and 512 and 1024 units respectively, whereas the third layer is also a fully connected layer with Sigmoid activation and 784 units for the MNIST dataset. The sum of squared differences between the outputs of the logistic units and the input pixel intensities is taken as the loss function and it is minimized during the training phase.

We intend to use the classifier of the existing architecture to our network, subjected to one minor change. Instead of using $9\times9$ kernels in the first convolutional layer and the subsequent capsule layer, we use $3\times3$ kernels, in order to capture the lower level features with the smallest localized area.
As for the reconstruction network shown in figure \ref{fig:capsnet}, we use an architecture with five deconvolution layers \cite{decon2010} (\textcolor{red}{explain deconvolution -hj}) and a fully connected layer. The first layer is the fully connected layer with ReLU activation and 6272 units. Then the output of the fully connected layer is reshaped in to $7\times7\times128$ in order to feed to the first deconvolution layer. This layer consists of 128 number of $3\times3$ kernels with $(1,1)$ sub sampling. Second deconvolution layer consists of 64 number of $3\times3$ kernels with $(2,2)$ sub sampling. Third deconvolution layer consists of 32 number of $3\times3$ kernels with $(2,2)$ sub sampling. Final convolution layer consists of one $3\times3$ kernel with $(1,1)$ sub sampling, resulting $28\times28\times1$ image for the EMNIST data set.
 We consider this architecture, as illustrated by figure \ref{fig:base}, to be the base model throughout this paper. 
 
\begin{figure}[h]
  \centering
  \includegraphics[scale=0.2]{figures/capsnet.png}
  \caption{\textbf{TextCap Model}: Base model for the character classification. This model surpass the previous results on handwritten character recognition. }

 \label{fig:base}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[scale=0.2]{figures/capsnet.png}
  \caption{\textbf{TextCap Decoder}: Decoder network for the character reconstruction. Input to this network is obtained by masking the DigitCaps layer of the TextCap classifier}

 \label{fig:decoder}
\end{figure}

\cite{sabour2017dynamic} already established that model in figure \ref{fig:capsnet} achieves state-of-the-art performance for the full MNIST dataset, with 6000 data points per training class. We evaluate the base model for its performance when the number of data points available is as low as 200 data points per training class.

\begin{figure}[h]
  \centering
  \includegraphics[scale=0.2]{figures/capsnet.png}
  \caption{\textbf{Original Model}: This is the original CapsNet model present in the original paper \cite{sabour2017dynamic}. }

 \label{fig:capsnet}
\end{figure}



==> relatedWork_capsnet.tex <==
\section{Capsule Networks and Dynamic Routing Algorithm}
\label{sect:related_caps}
A capsule is a group of neurons whose activity vectors represent not only the probability of existence of a certain entity, but a set of instantiation parameters \cite{hinton2011transforming}. The instantiation parameters can include pose (position, size, orientation), deformation, velocity, albedo, hue, texture and etc. \cite{sabour2017dynamic}. Hence, a capsule can be said to have the ability to learn a set of properties of a particular entity, rather than learning to detect the presence of that entity, similar to CNN. \jathu{rewrite}

Once pixel intensities have been converted into the outputs of a set of active, first-level capsules each of which produces an explicit representation of the pose of its visual entity. these low level capsules used to learn part-whole relationship and build up high level capsules.

An important notion in utilizing part-whole relationship for object recognition is that, even though the instantiation parameters for part entities and whole entities can vary for different inputs, the spatial relationship between a part entity and its whole entity remains static. Hence, part-whole relationship is viewpoint invariant \cite{hinton2011transforming}.

Consider that a capsules in layer $l$ learns part entities whereas the capsules in layer $l+1$ learns the whole entities, which are made from the part entities in layer $l$. Each output vector $u_i$ of layer $l$, represents the instantiation parameters of the part entity. capsules in layer $l+1$ learn the part-whole relationship and build a whole entity capsule $v_j$ from $u_i, i \in [N_l]$. where $N_l, N_{l+1}$ are the number of capsules in layer $l, l+1$ respectively.

% Capsules use high-dimensional coincidence filtering: a familiar object can be detected by looking for agreement between votes for its pose matrix. \cite{hinton2018matrix}

In the perspective of the capsule $j$, it can receive multiple predictions from the lower layer. Similarly, in the perspective of Capsule $i$, it has a choice of sending its output to multiple capsules in the higher layer. The fact that the output of a capsule outputs a more meaningful activity vector, rather than merely an activation value, allows the output to be dynamically routed to high level capsules which agree more with it. Such routing mechanisms are termed as \textit{Routing-by-agreement}.

\subsubsection{Dynamic Routing Algorithm}

part-whole spatial relationship between the capsule $i$ in the layer $l$ and the capsule $j$ in the layer $l+1$ is learned by the transformation matrix $W_{ij}$ during back propagation. Hence, from equation[\ref{eq:pred}], we can obtain a prediction for the existence and pose of the part entity in layer $l+1$ from $\hat{u}_{j|i}$. 

\begin{equation} \label{eq:pred}
\hat{u}_{j|i} = W_{ij} \times u_i
\end{equation}
\begin{equation} \label{eq:sum}
s_{j} = \sum_{i}^{} c_{ij}\hat{u}_{ij}
\end{equation}


$s_j$ can be interpreted as the weighted sum of predictions from the capsules in layer $l$. Hence, the output of the capsule $j$, $v_j$ can be calculated with the aid of $s_j$, according to eq[\ref{eq:vj}].  Squash function is used to keep the capsule vector within unit length while preserving orientation, so its length will represent the probability of the existence of an entity.

\begin{equation} \label{eq:vj}
v_{j} = \frac{||s_j||^2}{1+||s_j||^2} \frac{s_j}{||s_j||}
\end{equation}


The subsequent task is to route the outputs of the capsules in layer $l$ as the inputs of capsules in layer $l+1$. which requires to update $c_{ij}$ at each routing.

\begin{equation} \label{eq:softmax}
c_{ij} = \frac{exp(b_{ij})}{ \sum_{j}^{} exp(b_{ik})}
\end{equation}
\begin{equation} \label{eq:bij}
b_{ij} = b_{ij}+\hat{u}_{ij} \cdot v_{j}
\end{equation}
$b_{ij}$ is initialized to zero is to provide equal value to $c_{ij}$ in first routing. As the procedure progresses, the $c_{ij}$ will be eventually updated with $a_{ij} = \hat{u}_{ij} \cdot v_{j}$. here $a_{ij}$ corresponding to the argument between $v_j$ and $\hat{u}_{ij}$, hence routing by argument.
